Model-Driven Dataset Generation for Data-Driven Battery SOH Models

Estimating the State of Health (SOH) of batteries is crucial for ensuring the reliable operation of battery systems. Since there is no practical way to instantaneously measure it at run time, a model is required for its estimation. Recently, several data-driven SOH models have been proposed, whose accuracy heavily relies on the quality of the datasets used for their training. Since these datasets are obtained from measurements, they are limited in the variety of the charge/discharge profiles. To address this scarcity issue, we propose generating datasets by simulating a traditional battery model (e.g., a circuit-equivalent one). The primary advantage of this approach is the ability to use a simulatable battery model to evaluate a potentially infinite number of workload profiles for training the data-driven model. Furthermore, this general concept can be applied using any simulatable battery model, providing a fine spectrum of accuracy/complexity tradeoffs. Our results indicate that using simulated data achieves reasonable accuracy in SOH estimation, with a 7.2% error relative to the simulated model, in exchange for a 27X memory reduction and a =2000X speedup.

==> notes.tex <==
\subsection{Dataset}
This dataset presents data for 28 18650 LCO cells with 2.1 Ah capacity in seven groups. Five groups of cells were cycled at room temperature and the other two groups were cycled at 40°C. The dataset was recorded in 2014.

Cycling for each cell consisted of two types of charge/discharge cycles: Random Walk (RW) cycling and pulsed load characterization cycling. For each cell, after every set of 50 random walk cycles, a pulsed load characterization cycle was performed. In RW cycling, the current profile for both discharge and charge was changed every five minutes to a value randomly selected from the set of 0.5, 1, 1.5, 2, 2.5, 3, 3.5, or 4 A. In pulsed load cycling, the discharge profile consisted of a rest period of 20 minutes followed by a loading period of 10 minutes at 1 A. Randomized loads were applied during discharge in an effort to simulate more realistic usage.
